Computing Real Roots of Real Polynomials ... and now For Real!

Very recent work introduces an asymptotically fast subdivision algorithm, denoted ANewDsc, for isolating the real roots of a univariate real polynomial. The method combines Descartes' Rule of Signs to test intervals for the existence of roots, Newton iteration to speed up convergence against clusters of roots, and approximate computation to decrease the required precision. It achieves record bounds on the worst-case complexity for the considered problem, matching the complexity of Pan's method for computing all complex roots and improving upon the complexity of other subdivision methods by several magnitudes. In the article at hand, we report on an implementation of ANewDsc on top of the RS root isolator. RS is a highly efficient realization of the classical Descartes method and currently serves as the default real root solver in Maple. We describe crucial design changes within ANewDsc and RS that led to a high-performance implementation without harming the theoretical complexity of the underlying algorithm. With an excerpt of our extensive collection of benchmarks, available online at http://anewdsc.mpi-inf.mpg.de/, we illustrate that the theoretical gain in performance of ANewDsc over other subdivision methods also transfers into practice. These experiments also show that our new implementation outperforms both RS and mature competitors by magnitudes for notoriously hard instances with clustered roots. For all other instances, we avoid almost any overhead by integrating additional optimizations and heuristics.

==> preamble-arxiv.tex <==
%%% CUSTOMIZATIONS

\usepackage{cleveref}
\crefname{algocount}{Algorithm}{Algorithms}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{proof}{Proof}{Proofs}
\Crefname{figure}{Figure}{Figures}
\crefformat{equation}{#2(#1)#3}
\Crefformat{equation}{Equation #2(#1)#3}
\crefmultiformat{equation}{#2(#1)#3}{ and~#2(#1)#3}{, #2(#1)#3}{ and~#2(#1)#3}
\Crefmultiformat{equation}{Equations #2(#1)#3}{ and~#2(#1)#3}{, #2(#1)#3}{ and~#2(#1)#3}
\crefrangeformat{equation}{#3(#1)#4--#5(#2)#6}
\Crefrangeformat{equation}{Equations #3(#1)#4 to #5(#2)#6}
\crefformat{enumi}{#2(#1)#3}
\crefformat{enumii}{#2(#1)#3}
\crefformat{enumiii}{#2(#1)#3}
\crefformat{enumiv}{#2(#1)#3}
%% from http://tex.stackexchange.com/questions/125558/what-is-the-dry-way-to-get-theorem-1a
\makeatletter
\def\@itemref#1#2:#3\relax{#1{#2}\;\cref{#2:#3}}
\newcommand{\itemref}[1]{\@itemref\cref#1\relax}
\newcommand{\Itemref}[1]{\@itemref\Cref#1\relax}
\makeatother
\crefname{lemma}{Lemma}{Lemmas}
% \crefname{section}{Sec.}{Secs.}
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefformat{appendix}{#2#1#3}

% \usepackage{multibib}
% \newcites{app}{Additional References}

\newcommand{\ignore}[1]{}

\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\rs}{\textsc{Rs}\xspace}
\newcommand{\isolate}{\textsc{Isolate}\xspace}
\newcommand{\lgp}{\textsc{Lgp}\xspace}
% \newcommand{\sep}{\operatorname{sep}}
\newcommand{\sep}{\ensuremath{\sigma}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\tO}{\smash{\tilde{O}}}
\DeclareMathOperator{\LOG}{\ensuremath{\operatorname{log\mathllap{\raisebox{1.35ex}{\rule{0.95em}{0.08ex}}\hspace{0.025em}}}}}
\DeclareMathOperator{\crampedLOG}{\ensuremath{\operatorname{log\mathllap{\raisebox{0.95ex}{\rule{0.65em}{0.06ex}}\hspace{0.025em}}}}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{task}{Task}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}

\DeclarePairedDelimiter\set{\{}{\}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\sumnorm{\lVert}{\rVert_1}
\DeclarePairedDelimiter\infnorm{\lVert}{\rVert_\infty}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}


\definecolor{badcolor}{named}{DarkRed}
\definecolor{goodcolor}{named}{Green}
\newcommand{\bad}[1]{\textcolor{badcolor}{#1}}
\newcommand{\better}[1]{\textcolor{badcolor!66.667!goodcolor}{#1}}
\newcommand{\good}[1]{\textcolor{badcolor!33.333!goodcolor}{#1}}
\newcommand{\great}[1]{\textcolor{goodcolor}{#1}}

\usepackage{array,tabularx,multirow}
% \usepackage{longtable}
% \setlength\LTleft{0pt}
% \setlength\LTright{0pt}
\addtolength{\tabcolsep}{-0.25ex}

% from: http://tex.stackexchange.com/questions/144434/re-newing-a-column-type
\newcommand\undefcolumntype[1]{\expandafter\let\csname NC@find@#1\endcsname\relax}
\newcommand\forcenewcolumntype[1]{\undefcolumntype{#1}\newcolumntype{#1}}

\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\usepackage{booktabs}

\usepackage{multirow}
\usepackage{numprint}
\usepackage{array}
\npdecimalsign{.}
\nprounddigits{1}
% \newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{\!\!}|}
\forcenewcolumntype{N}{n{5}{2}}
\newcolumntype{S}{n{3}{1}}
%\usepackage{pgfplots}

\newcommand{\error}{\textcolor{badcolor}{\emph{err}}}
\newcommand{\timeout}{\textcolor{badcolor}{\strut\clap{$*$}\phantom{\scalebox{0.5}{.}0}\strut}}
\renewcommand{\timeout}{\textcolor{badcolor}{\strut\emph{\textgreater~600}\strut}}
% \newcommand{\tablesize}{\fontsize{7pt}{8.2pt}\selectfont}
% \newcommand{\captionfont}{\fontsize{6.5pt}{8pt}\selectfont}
\newcommand{\tablesize}{}
%% \newcommand{\captionfont}{}
\newlength{\timecolwidth}
\setlength{\timecolwidth}{\maxof{\widthof{\tablesize 000.0}}{\widthof{\tablesize{\textsc{ADsc}}}}}
\setlength{\timecolwidth}{\maxof{\widthof{\tablesize\timeout}}{\widthof{\tablesize{\textsc{ADsc}}}}}
\newlength{\degcolwidth}
% \setlength{\degcolwidth}{\widthof{\tablesize\itshape10000}}
\setlength{\degcolwidth}{\widthof{\tablesize 10000}}
\newlength{\btscolwidth}
\setlength{\btscolwidth}{\widthof{\tablesize\quad 100000}}
\newcolumntype{T}{>{\raggedleft\arraybackslash}p{\timecolwidth}}
% \newcolumntype{D}{>{\raggedleft\arraybackslash\itshape}p{\degcolwidth}}
% \newcolumntype{B}{>{\raggedleft\arraybackslash\itshape}p{\btscolwidth}}
\newcolumntype{D}{>{\raggedleft\arraybackslash}p{\degcolwidth}}
\newcolumntype{B}{>{\raggedleft\arraybackslash}p{\btscolwidth}}

\newcommand{\vcenterwithline}[2]{%
  \setlength{\dimen0}{.5\baselineskip * (#1 - 2)}%
  \settoheight{\dimen1}{0}%
  \settowidth{\dimen2}{#2}%
  \multirow{#1}{*}{%
      #2%
      \hspace{-0.5\dimen2}\hspace{-0.5\lightrulewidth}%
      \raisebox{\baselineskip}[0pt][0pt]{\rule{\lightrulewidth}{\dimen0}}%
      \hspace{-\lightrulewidth}%
      \raisebox{-\baselineskip + \dimen1 - \dimen0}[0pt][0pt]{\rule{\lightrulewidth}{\dimen0}}%
      \hspace{0.5\dimen2}\hspace{-0.5\lightrulewidth}%
      % \raisebox{-\baselineskip}[0pt][0pt]{\rule{.5pt}{\dimen0}}%
      % \makebox[\widthof{#2}]{\rule{.5pt}{\dimen0}}\\
    % }%
  }%
}

%% \usepackage{hanging}
%% \setlength{\textfloatsep}{0.75em plus 0.75em minus 0.75ex}
%% \setlength{\dbltextfloatsep}{1ex}
%% \setlength{\floatsep}{1ex plus 1em}
%% \setlength{\intextsep}{0.75em plus 0.75em minus 0.75ex}
%% \setlength{\belowcaptionskip}{0.5ex plus 0.5ex minus 0.5ex}
\floatstyle{boxed}
\newfloat{algorithm}{htp}{algorithm}[section]
\let\oldalgorithm\algorithm
\renewcommand{\algorithm}[1][]{\oldalgorithm[#1]\raggedright}
\newcounter{algocount}
% \newcommand{\algtitle}[1]{\refstepcounter{algocount}\textsc{\textbf{Algorithm \ref*{algo:#1}: #1}}\label{algo:#1}\smallskip}
% \newcommand{\algspecialtitle}[2]{\refstepcounter{algocount}\textsc{\textbf{Algorithm \ref*{algo:#2}: #1}}\label{algo:#2}\smallskip}
\newcommand{\algtitle}[1]{\refstepcounter{algocount}\textbf{Algorithm \ref*{algo:#1}: #1}\label{algo:#1}\smallskip}
\newcommand{\algspecialtitle}[2]{\refstepcounter{algocount}\textbf{Algorithm \ref*{algo:#2}: #1}\label{algo:#2}\smallskip}
\newcommand{\alginput}[1]{\par\noindent\hangindent=3.47em\hangafter=1\textsc{Input:} #1\smallskip}
\newcommand{\algoutput}[1]{\par\noindent\hangindent=4.47em\hangafter=1\textsc{Output:} #1\smallskip}
\newcommand{\algreports}[1]{\par\noindent\hangindent=4.47em\hangafter=1\textsc{Reports:} #1\smallskip}
\newlist{algolist}{itemize}{2}
\setlist[algolist,1]{label=\textbullet, nosep, labelindent=0em, leftmargin=1.em, after=\smallskip}
\setlist[algolist,2]{label=$\triangleright$, nosep, labelindent=0em, leftmargin=1.em}

\makeatletter
% % unnumbered lemmata
% \def\@begintheorem#1#2{%
%     \parskip 0pt % GM July 2000 (for tighter spacing)
%     \trivlist
%     \item[%
%         \hskip 10\p@
%         \hskip \labelsep
%         {{\sc #1}.}%
%     ]
%     \it
% }

\newcommand{\flexvspace}{\vspace{1em minus 1ex}}
\def\flexvspacenoindent{%
  \flexvspace
  \par\noindent%
  \@ifnextchar\par\@gobble\relax%
}
\let\oldparagraph\paragraph
\renewcommand{\paragraph}[1]{\oldparagraph{#1}}
\makeatother

\providecommand{\TODO}[1]{\textcolor{red}{[\textsc{TODO: }{\sf #1}]}}
\providecommand{\TODO}[1]{\unskip}
\providecommand{\Michael}[1]{\unskip}
\providecommand{\Fabrice}[1]{\unskip}
\providecommand{\Alex}[1]{\unskip}
\providecommand{\Reviewer}[1]{\unskip}

\providecommand{\shortversion}[1]{#1}
\providecommand{\fullversion}[1]{#1}

